Discovering and Achieving Goals via World Models

How can artificial agents learn to solve many diverse tasks in complex visual environments in the absence of any supervision? We decompose this question into two problems: discovering new goals and learning to reliably achieve them. We introduce Latent Explorer Achiever (LEXA), a unified solution to these that learns a world model from image inputs and uses it to train an explorer and an achiever policy from imagined rollouts. Unlike prior methods that explore by reaching previously visited states, the explorer plans to discover unseen surprising states through foresight, which are then used as diverse targets for the achiever to practice. After the unsupervised phase, LEXA solves tasks specified as goal images zero-shot without any additional learning. LEXA substantially outperforms previous approaches to unsupervised goal-reaching, both on prior benchmarks and on a new challenging benchmark with a total of 40 test tasks spanning across four standard robotic manipulation and locomotion domains. LEXA further achieves goals that require interacting with multiple objects in sequence. Finally, to demonstrate the scalability and generality of LEXA, we train a single general agent across four distinct environments. Code and videos at https://orybkin.github.io/lexa/

==> figures/ablations/figure.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.33\linewidth, valign=t]{figures/curve_plots/bin_sorting_ablation_curve_cropped.pdf} $\,$
\includegraphics[width=0.65\linewidth, valign=t]{figures/heatmaps/bin_sorting_ablation_hmap_cropped.pdf}
\caption{\textbf{Ablations.} Testing different components of LEXA with temporal distances on RoboBins. We observe that training a separate exploration policy is crucial for most tasks, as the agent never discovers them in the \textit{no explorer} version. Training temporal distance on negative samplies significantly speeds up learning, and both negative sampling and training in imagination as opposed to real data is important for performance on the hardest tasks.}
\label{fig:ablations}
\end{figure}


==> figures/coincidental_exploration/bin_figure.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.8\linewidth, valign=t]{figures/coincidental_exploration/Bin_expl_sel_tasks_bplot.pdf}
% \vspace{-0.1in}
\caption{Coincidental exploration success for the RoboBin environment. The bar plot shows the number of collected trajectories that coincidentally satisfy the success criterion of the goal images used for evaluation, when about 1e5 trajectories have been collected in total. \todo refine caption}
\label{fig:executions}
\end{figure}

==> figures/prior/figure.tex <==
\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{prior/prior}
\caption{Performance on prior benchmarks. LEXA outperforms all prior goal image agents.}
\label{fig:prior}
\end{figure}

==> tables/prior.tex <==
\begin{table}[b]
\centering
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method} & \textbf{Visual Pusher} & \textbf{Visual Pickup} &  \textbf{DMC Random Goals} & \textbf{DMC Tasks} \\
\midrule
RIG \cite{nair2018imagined} & 0.077 & 0.037 & --- & --- \\
SkewFit \cite{pong2019skewfit} & 0.049 & 0.018 & --- & --- \\
HER \cite{andrychowicz2017hindsight} & 0.075 & 0.035 & --- & --- \\
DISCERN \cite{warde2018discern} & --- & --- & 55.3\% & --- \\
Plan2Explore \citep{sekar2020plan2explore} & --- & --- & --- & 686 \\
DrQv2 (oracle) \rlap{\cite{yarats2021drqv2}} & --- & --- & --- & 944 \\
\midrule
LEXA + cosine & --- & --- & \textbf{70.5\%} & \textbf{910} \\
LEXA + temporal & \textbf{0.023} & \textbf{0.014} & --- & --- \\
\bottomrule
\end{tabular}
\vspace{1ex}
\caption{Performance on prior benchmarks. LEXA outperforms all prior goal image agents.}
\label{tab:prior}
\end{table}

